MiniScope: Automated UI Exploration and Privacy Inconsistency Detection of MiniApps via Two-phase Iterative Hybrid Analysis

The advent of MiniApps, operating within larger SuperApps, has revolutionized user experiences by offering a wide range of services without the need for individual app downloads. However, this convenience has raised significant privacy concerns, as these MiniApps often require access to sensitive data, potentially leading to privacy violations. Despite existing privacy regulations and platform guidelines, there is a lack of effective mechanisms to safeguard user privacy fully. To address this critical gap, we introduce MiniScope, a novel two-phase hybrid analysis approach, specifically designed for the MiniApp environment. This approach overcomes the limitations of existing static analysis techniques by incorporating UI transition states analysis, cross-package callback control flow resolution, and automated iterative UI exploration. This allows for a comprehensive understanding of MiniApps' privacy practices, addressing the unique challenges of sub-package loading and event-driven callbacks. Our empirical evaluation of over 120K MiniApps using MiniScope demonstrates its effectiveness in identifying privacy inconsistencies. The results reveal significant issues, with 5.7% of MiniApps over-collecting private data and 33.4% overclaiming data collection. We have responsibly disclosed our findings to 2,282 developers, receiving 44 acknowledgments. These findings emphasize the urgent need for more precise privacy monitoring systems and highlight the responsibility of SuperApp operators to enforce stricter privacy measures.

==> reference <==
@article{Kumar_2018,
    title={Advances in Intrusion Detection and Prevention Techniques: A Survey},
    volume={6},
    ISSN={2162-237X},
    url={http://dx.doi.org/10.5815/ijcnis.2018.06.01},
    DOI={10.5815/ijcnis.2018.06.01},
    journal={International Journal of Computer Network and Information Security},
    publisher={IJCNS},
    author={Kumar, Vijay and Arya, Shikha and Gupta, Vinesh Kumar},
    year={2018},
    month={Apr},
    pages={1–13}
}

@inproceedings{yang2022cross,
  title={Cross Miniapp Request Forgery: Root Causes, Attacks, and Vulnerability Detection},
  author={Yang, Yuqing and Zhang, Yue and Lin, Zhiqiang},
  booktitle={Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security},
  pages={3079--3092},
  year={2022}
}

@Misc{wechatshopping,
    title = "eCommerce SaaS solution by WeChat: a complete guide",
    howpublished = {\url{https://wechatwiki.com/wechat-resources/wechat-mini-shop-ecommerce-solution/}},
    year = 2022,
}

@article{rao2021impulsive,
  title={Impulsive purchasing and luxury brand loyalty in WeChat Mini Program},
  author={Rao, Qianhui and Ko, Eunju},
  journal={Asia Pacific Journal of Marketing and Logistics},
  year={2021},
  publisher={Emerald Publishing Limited}
}

@article{qian2021did,
  title={How did Wuhan residents cope with a 76-day lockdown?},
  author={Qian, Yue and Hanser, Amy},
  journal={Chinese Sociological Review},
  volume={53},
  number={1},
  pages={55--86},
  year={2021},
  publisher={Taylor \& Francis}
}

@Misc{whitepaper2021,
    title = "White Paper on Internet Development of MiniApps in 2021",
    howpublished = {\url{https://aldzs.com/viewpointarticle?id=16175}},
    year = 2022,
}

@inproceedings{hao2018analysis,
  title={Analysis of the development of WeChat mini program},
  author={Hao, Lei and Wan, Fucheng and Ma, Ning and Wang, Yicheng},
  booktitle={Journal of Physics: Conference Series},
  volume={1087},
  number={6},
  pages={062040},
  year={2018},
  organization={IOP Publishing}
}

@article{yang2023sok,
  title={{SoK: Decoding the Super App Enigma: The Security Mechanisms, Threats, and Trade-offs in OS-alike Apps}},
  author={Yang, Yuqing and Wang, Chao and Zhang, Yue and Lin, Zhiqiang},
  journal={{arXiv preprint}},
  year={2023}
}

@Misc{GDPR,
    title = "General Data Protection Regulation",
    howpublished = {\url{https://commission.europa.eu/law/law-topic/data-protection_en}},
    year = 2022,
}

@Misc{CCPA,
    title = "California Consumer Privacy Act",
    howpublished = {\url{https://oag.ca.gov/privacy/ccpa}},
    year = 2022,
}

@Misc{APPI,
    title = "Act on the Protection of Personal Information",
    howpublished = {\url{https://www.ppc.go.jp/}},
    year = 2022,
}

@Misc{PDPA,
    title = "Personal Data Protection Act",
    howpublished = {\url{https://www.pdpc.gov.sg/}},
    year = 2022,
}

@inproceedings{cheng2019exploratory,
  title={An exploratory analysis of travel-related WeChat mini program usage: affordance theory perspective},
  author={Cheng, Ao and Ren, Gang and Hong, Taeho and Nam, Kichan and Koo, Chulmo},
  booktitle={Information and Communication Technologies in Tourism 2019: Proceedings of the International Conference in Nicosia, Cyprus, January 30--February 1, 2019},
  pages={333--343},
  year={2019},
  organization={Springer}
}

@article{zhang2021measurement,
  title={A measurement study of wechat mini-apps},
  author={Zhang, Yue and Turkistani, Bayan and Yang, Allen Yuqing and Zuo, Chaoshun and Lin, Zhiqiang},
  journal={ACM SIGMETRICS Performance Evaluation Review},
  volume={49},
  number={1},
  pages={19--20},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@inproceedings{wang2023taintmini,
  title={TAINTMINI: Detecting Flow of Sensitive Data in Mini-Programs with Static Taint Analysis},
  author={Wang, Chao and Ko, Ronny and Zhang, Yue and Yang, Yuqing and Lin, Zhiqiang},
  booktitle={Proceedings of the 45th International Conference on Software Engineering},
  year={2023}
}

@inproceedings{lu2020demystifying,
  title={Demystifying resource management risks in emerging mobile app-in-app ecosystems},
  author={Lu, Haoran and Xing, Luyi and Xiao, Yue and Zhang, Yifan and Liao, Xiaojing and Wang, XiaoFeng and Wang, Xueqiang},
  booktitle={Proceedings of the 2020 ACM SIGSAC conference on computer and communications Security},
  pages={569--585},
  year={2020}
}

@inproceedings{shezan2023chkplug,
  title={CHKPLUG: Checking GDPR Compliance of WordPress Plugins via Cross-language Code Property Graph.},
  author={Shezan, Faysal Hossain and Su, Zihao and Kang, Mingqing and Phair, Nicholas and Thomas, Patrick William and van Dam, Michelangelo and Cao, Yinzhi and Tian, Yuan},
  booktitle={NDSS},
  year={2023}
}

@inproceedings{zhao2022ca4p483,
    title = "A Fine-grained Chinese Software Privacy Policy Dataset for Sequence Labeling and Regulation Compliant Identification",
    author = "Zhao, Kaifa and 
      Yu, Le and 
      Zhou, Shiyao and 
      Li, Jing and 
      Luo, Xiapu and 
      Chiu, Yat Fei Aemon and 
      Liu, Yutong",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2022",
    publisher = "Association for Computational Linguistics",
}

@inproceedings{zhang2022identity,
  title={Identity Confusion in $\{$WebView-based$\}$ Mobile App-in-app Ecosystems},
  author={Zhang, Lei and Zhang, Zhibo and Liu, Ancong and Cao, Yinzhi and Zhang, Xiaohan and Chen, Yanjun and Zhang, Yuan and Yang, Guangliang and Yang, Min},
  booktitle={31st USENIX Security Symposium (USENIX Security 22)},
  pages={1597--1613},
  year={2022}
}

@inproceedings{liu2020industry,
  title={Industry practice of javascript dynamic analysis on wechat mini-programs},
  author={Liu, Yi and Xie, Jinhui and Yang, Jianbo and Guo, Shiyu and Deng, Yuetang and Li, Shuqing and Wu, Yechang and Liu, Yepang},
  booktitle={Proceedings of the 35th IEEE/ACM International Conference on Automated Software Engineering},
  pages={1189--1193},
  year={2020}
}

@inproceedings{sen2013jalangi,
  title={Jalangi: A selective record-replay and dynamic analysis framework for JavaScript},
  author={Sen, Koushik and Kalasapur, Swaroop and Brutch, Tasneem and Gibbs, Simon},
  booktitle={Proceedings of the 2013 9th Joint Meeting on Foundations of Software Engineering},
  pages={488--498},
  year={2013}
}

@inproceedings{li2019find,
  title={How to Find It Better? Cross-Learning for WeChat Mini Programs},
  author={Li, He and Liu, Zhiqiang and Xu, Sheng and Lin, Zhiyuan and Chen, Xiangqun},
  booktitle={Proceedings of the 28th ACM International Conference on Information and Knowledge Management},
  pages={2753--2761},
  year={2019}
}

@inproceedings{wang2022characterizing,
  title={Characterizing and detecting bugs in WeChat mini-programs},
  author={Wang, Tao and Xu, Qingxin and Chang, Xiaoning and Dou, Wensheng and Zhu, Jiaxin and Xie, Jinhui and Deng, Yuetang and Yang, Jianbo and Yang, Jiaheng and Wei, Jun and others},
  booktitle={Proceedings of the 44th International Conference on Software Engineering},
  pages={363--375},
  year={2022}
}

@inproceedings{andow2020actions,
  title={Actions speak louder than words:$\{$Entity-Sensitive$\}$ privacy policy and data flow analysis with $\{$PoliCheck$\}$},
  author={Andow, Benjamin and Mahmud, Samin Yaseer and Whitaker, Justin and Enck, William and Reaves, Bradley and Singh, Kapil and Egelman, Serge},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={985--1002},
  year={2020}
}

@inproceedings{harkous2018polisis,
  title={Polisis: Automated analysis and presentation of privacy policies using deep learning},
  author={Harkous, Hamza and Fawaz, Kassem and Lebret, R{\'e}mi and Schaub, Florian and Shin, Kang G and Aberer, Karl},
  booktitle={27th USENIX Security Symposium (USENIX Security 18)},
  pages={531--548},
  year={2018}
}

@inproceedings{andow2019policylint,
  title = {{Policylint: Investigating Internal Privacy Policy Contradictions on Google Play}},
  author={Andow, Benjamin and Mahmud, Samin Yaseer and Wang, Wenyu and Whitaker, Justin and Enck, William and Reaves, Bradley and Singh, Kapil and Xie, Tao},
  booktitle={28th USENIX security symposium (USENIX security 19)},
  pages={585--602},
  year={2019}
}

@article{wang2023gpt,
  title={Gpt-ner: Named entity recognition via large language models},
  author={Wang, Shuhe and Sun, Xiaofei and Li, Xiaoya and Ouyang, Rongbin and Wu, Fei and Zhang, Tianwei and Li, Jiwei and Wang, Guoyin},
  journal={arXiv preprint arXiv:2304.10428},
  year={2023}
}

@Misc{CPPA,
    title = {{Consumer Privacy Protection Act}},
    howpublished = {\url{https://ised-isde.canada.ca/site/innovation-better-canada/en/consumer-privacy-protection-act}},
    year = 2022,
}


@Misc{Wechat_privacypolicy,
    title = {{WECHAT PRIVACY POLICY}},
    howpublished = {\url{https://www.wechat.com/en/privacy_policy.html}},
    year = 2023,
}

@Misc{Wechat_API_Documentation,
    title = {{WeChat API Documentation}},
    howpublished = {\url{https://developers.weixin.qq.com/miniprogram/en/dev/api/}},
    year = 2023,
}

@Misc{Wechat_risk1,
    title = {{Should We Chat? Privacy in the WeChat Ecosystem}},
    howpublished = {\url{https://citizenlab.ca/2023/06/privacy-in-the-wechat-ecosystem-full-report/}},
    year = 2023,
}


@Misc{Wechat_risk2,
    title = {{First Major Analysis of WeChat Ecosystem Network Requests Finds Privacy Gaps, Undisclosed Data Sharing}},
    howpublished = {\url{https://www.cpomagazine.com/data-privacy/first-major-analysis-of-wechat-ecosystem-network-requests-finds-privacy-gaps-undisclosed-data-sharing/}},
    year = 2023,
}

@misc{wang2023uncovering,
      title={{Uncovering and Exploiting Hidden APIs in Mobile Super Apps}}, 
      author={Chao Wang and Yue Zhang and Zhiqiang Lin},
      year={2023},
      eprint={2306.08134},
      archivePrefix={{arXiv}}
}

@Misc{chatgpt,
    title = {{ChatGPT}},
    howpublished = {\url{https://chat.openai.com}},
    year = 2022,
}

@article{zhoupolicycomp,
  title={POLICYCOMP: Counterpart Comparison of Privacy Policies Uncovers Overbroad Personal Data Collection Practices},
  author={Zhou, Lu and Wei, Chengyongxiao and Zhu, Tong and Chen, Guoxing and Zhang, Xiaokuan and Du, Suguo and Cao, Hui and Zhu, Haojin}
}

@Misc{wxappUnpacker,
  title = "{wxappUnpacker}",
  author="{xdmjun}",
  note = {\url{https://github.com/xdmjun/wxappUnpacker}},
  year=2023
}

@Misc{unveilr,
  title = "{unveilr}",
  author="{r3x5ur}",
  note = {\url{https://github.com/r3x5ur/unveilr}},
  year=2023
}

@inproceedings{yamaguchi2014modeling,
  title={Modeling and discovering vulnerabilities with code property graphs},
  author={Yamaguchi, Fabian and Golde, Nico and Arp, Daniel and Rieck, Konrad},
  booktitle={2014 IEEE Symposium on Security and Privacy},
  pages={590--604},
  year={2014},
  organization={IEEE}
}

@article{yang2018wtg,
  title={Static window transition graphs for Android},
  author={Yang, Shengqian and Wu, Haowei and Zhang, Hailong and Wang, Yan and Swaminathan, Chandrasekar and Yan, Dacong and Rountev, Atanas},
  journal={Automated Software Engineering},
  volume={25},
  pages={833--873},
  year={2018},
  publisher={Springer}
}

@inproceedings{dong2018frauddroid,
  title={Frauddroid: Automated ad fraud detection for android apps},
  author={Dong, Feng and Wang, Haoyu and Li, Li and Guo, Yao and Bissyand{\'e}, Tegawend{\'e} F and Liu, Tianming and Xu, Guoai and Klein, Jacques},
  booktitle={Proceedings of the 2018 26th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
  pages={257--268},
  year={2018}
}

@inproceedings{liu2022promal,
  title={ProMal: precise window transition graphs for android via synergy of program analysis and machine learning},
  author={Liu, Changlin and Wang, Hanlin and Liu, Tianming and Gu, Diandian and Ma, Yun and Wang, Haoyu and Xiao, Xusheng},
  booktitle={Proceedings of the 44th International Conference on Software Engineering},
  pages={1755--1767},
  year={2022}
}

@inproceedings{yang2015ccfg,
  title={Static control-flow analysis of user-driven callbacks in Android applications},
  author={Yang, Shengqian and Yan, Dacong and Wu, Haowei and Wang, Yan and Rountev, Atanas},
  booktitle={2015 IEEE/ACM 37th IEEE International Conference on Software Engineering},
  volume={1},
  pages={89--99},
  year={2015},
  organization={IEEE}
}

@inproceedings{ling2022arethey,
author = {Ling, Yuxi and Wang, Kailong and Bai, Guangdong and Wang, Haoyu and Dong, Jin Song},
title = {Are they Toeing the Line? Diagnosing Privacy Compliance Violations among Browser Extensions},
year = {2023},
isbn = {9781450394758},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3551349.3560436},
doi = {10.1145/3551349.3560436},
abstract = {Browser extensions have emerged as integrated characteristics in modern browsers, with the aim to boost the online browsing experience. Their advantageous position between a user and the Internet endows them with easy access to the user’s sensitive data, which has raised mounting privacy concerns from both legislators and extension users. In this work, we propose an end-to-end approach to automatically diagnosing the privacy compliance violations among extensions. It analyzes the compliance of privacy policy versus regulation requirements and their actual privacy-related practices during runtime. This approach can serve the extension users, developers and store operators as an efficient and practical detection mechanism for privacy compliance violations. Our approach utilizes the state-of-the-art language processing model BERT for annotating the policy texts, and a hybrid technique to analyze an extension’s source code and runtime behavior. To facilitate the model training, we construct a corpus named PrivAud-100 which contains 100 manually annotated privacy policies. Our large-scale diagnostic evaluation reveals that the vast majority of existing extensions suffer from privacy non-compliance issues. Around 92\% of them have at least one violation of either their privacy policies or data collection practices. Based on our findings, we further propose an index to facilitate the filtering and identification of privacy-incompliant extensions with high accuracy&nbsp;(over 90\%). Our work should raise the awareness of extension users, service providers, and platform operators, and encourage them to implement solutions toward better privacy compliance. To facilitate future research in this area, we have released our dataset, corpus and analyzer.},
booktitle = {Proceedings of the 37th IEEE/ACM International Conference on Automated Software Engineering},
articleno = {10},
numpages = {12},
location = {Rochester, MI, USA},
series = {ASE '22}
}

@inproceedings{yang2022permdroid,
  title={PermDroid: automatically testing permission-related behaviour of Android applications},
  author={Yang, Shuaihao and Zeng, Zigang and Song, Wei},
  booktitle={Proceedings of the 31st ACM SIGSOFT International Symposium on Software Testing and Analysis},
  pages={593--604},
  year={2022}
}

@Misc{frida,
  title = "{Frida}",
  author="{frida}",
  note = {\url{https://frida.re/}},
  year=2023
}

@Misc{minidroid,
  title = "{MiniScope}",
  author="{ShenaoW}",
  note = {\url{https://github.com/ShenaoW/MiniScope}},
  year=2023
}

@Misc{online-form,
    title = {Online Documentation},
    author={Anonymous},
    howpublished = {\url{https://docs.google.com/spreadsheets/d/1l3P7D9kIRlDiR97ndGaa8xMLXooshIaQa0peYK2kV78/edit?usp=sharing}},
    year = 2023,
}

@Misc{appium,
  title = "{appium}",
  author="{appium}",
  note = {\url{https://github.com/appium/appium}},
  year=2023
}

@Misc{objection,
  title = "{objection}",
  author="{sensepost}",
  note = {\url{https://github.com/sensepost/objection}},
  year=2023
}

@Misc{w3c,
  title = "{MiniApp Standardization White Paper}",
  author="{W3C}",
  note = {\url{https://www.w3.org/TR/mini-app-white-paper}},
  year=2023
}

@Misc{subpackaging,
  title = "{MiniApp Subpackaging}",
  author="{W3C}",
  note = {\url{https://www.w3.org/TR/mini-app-white-paper/\#subpackaging}},
  year=2023
}

@article{zhang2023spochecker,
  title={Understanding Privacy Over-collection in WeChat Sub-app Ecosystem},
  author={Zhang, Xiaohan and Wang, Yang and Zhang, Xin and Huang, Ziqi and Zhang, Lei and Yang, Min},
  journal={arXiv preprint arXiv:2306.08391},
  year={2023}
}

@article{wang2023doasyousay,
  author={Wang, Yin and Fan, Ming and Liu, Junfeng and Tao, Junjie and Jin, Wuxia and Wang, Haijun and Xiong, Qi and Liu, Ting},
  journal={IEEE Transactions on Software Engineering}, 
  title={Do as You Say: Consistency Detection of Data Practice in Program Code and Privacy Policy in Mini-App}, 
  year={2024},
  volume={},
  number={},
  pages={1-23},
  keywords={Privacy;Codes;Social networking (online);Message services;Data privacy;Regulation;Operating systems;Smart phones;Prompt engineering;Protection;Mini-app;mini-program;privacy;consistency compliance detection;data flow analysis;prompt engineering},
  doi={10.1109/TSE.2024.3479288}
}

@inproceedings{meng2023wemint,
  title={Wemint: Tainting Sensitive Data Leaks in WeChat Mini-Programs},
  author={Meng, Shi and Wang, Liu and Wang, Shenao and Wang, Kailong and Xiao, Xusheng and Bai, Guangdong and Wang, Haoyu},
  booktitle={2023 38th IEEE/ACM International Conference on Automated Software Engineering (ASE)},
  pages={1403--1415},
  year={2023},
  organization={IEEE}
}

@article{li2023minitracker,
  title={MiniTracker: Large-Scale Sensitive Information Tracking in Mini Apps},
  author={Li, Wei and Yang, Borui and Ye, Hangyu and Xiang, Liyao and Tao, Qingxiao and Wang, Xinbing and Zhou, Chenghu},
  journal={IEEE Transactions on Dependable and Secure Computing},
  year={2023},
  publisher={IEEE}
}



@inproceedings{ma2018empirical,
  title={Empirical study on the Wechat Mini Program acceptance based on UTA UT model take the pearl river delta as an example},
  author={Ma, Lijun and Wang, Lan and Jiang, Entao},
  booktitle={2018 15th International Conference on Service Systems and Service Management (ICSSSM)},
  pages={1--6},
  year={2018},
  organization={IEEE}
}

@inproceedings{zhang2023small,
  title={A Small Leak Will Sink Many Ships: Vulnerabilities Related to mini-programs Permissions},
  author={Zhang, Jianyi and Yang, Leixin and Han, Yuyang and Xiang, Zixiao and Hei, Xiali},
  booktitle={2023 IEEE 47th Annual Computers, Software, and Applications Conference (COMPSAC)},
  pages={595--606},
  year={2023},
  organization={IEEE}
}

@article{zhang2023dont,
  title={Don't Leak Your Keys: Understanding, Measuring, and Exploiting the AppSecret Leaks in Mini-Programs},
  author={Zhang, Yue and Yang, Yuqing and Lin, Zhiqiang},
  journal={arXiv preprint arXiv:2306.08151},
  year={2023}
}

@article{baskaran2023measuring,
  title={Measuring the Leakage and Exploitability of Authentication Secrets in Super-apps: The WeChat Case},
  author={Baskaran, Supraja and Zhao, Lianying and Mannan, Mohammad and Youssef, Amr},
  journal={arXiv preprint arXiv:2307.09317},
  year={2023}
}

@inproceedings{meng2023wemint,
  title={Wemint: Tainting Sensitive Data Leaks in WeChat Mini-Programs},
  author={Meng, Shi and Wang, Liu and Wang, Shenao and Wang, Kailong and Xiao, Xusheng and Bai, Guangdong and Wang, Haoyu},
  booktitle={2023 38th IEEE/ACM International Conference on Automated Software Engineering (ASE)},
  pages={1403--1415},
  year={2023},
  organization={IEEE}
}

@inproceedings{slavin2016toward,
  title={Toward a framework for detecting privacy policy violations in android application code},
  author={Slavin, Rocky and Wang, Xiaoyin and Hosseini, Mitra Bokaei and Hester, James and Krishnan, Ram and Bhatia, Jaspreet and Breaux, Travis D and Niu, Jianwei},
  booktitle={Proceedings of the 38th International Conference on Software Engineering},
  pages={25--36},
  year={2016}
}

@inproceedings{wang2018guileak,
  title={Guileak: Tracing privacy policy claims on user input data for android applications},
  author={Wang, Xiaoyin and Qin, Xue and Hosseini, Mitra Bokaei and Slavin, Rocky and Breaux, Travis D and Niu, Jianwei},
  booktitle={Proceedings of the 40th International Conference on Software Engineering},
  pages={37--47},
  year={2018}
}

@inproceedings{nan2015uipicker,
  title={$\{$UIPicker$\}$:$\{$User-Input$\}$ Privacy Identification in Mobile Applications},
  author={Nan, Yuhong and Yang, Min and Yang, Zhemin and Zhou, Shunfan and Gu, Guofei and Wang, XiaoFeng},
  booktitle={24th USENIX Security Symposium (USENIX Security 15)},
  pages={993--1008},
  year={2015}
}

@inproceedings{bui2023detection,
  title={Detection of inconsistencies in privacy practices of browser extensions},
  author={Bui, Duc and Tang, Brian and Shin, Kang G},
  booktitle={2023 IEEE Symposium on Security and Privacy (SP)},
  pages={2780--2798},
  year={2023},
  organization={IEEE}
}

@inproceedings{ling2022they,
  title={Are they toeing the line? diagnosing privacy compliance violations among browser extensions},
  author={Ling, Yuxi and Wang, Kailong and Bai, Guangdong and Wang, Haoyu and Dong, Jin Song},
  booktitle={Proceedings of the 37th IEEE/ACM International Conference on Automated Software Engineering},
  pages={1--12},
  year={2022}
}

@inproceedings{andow2020actions,
  title={Actions speak louder than words:$\{$Entity-Sensitive$\}$ privacy policy and data flow analysis with $\{$PoliCheck$\}$},
  author={Andow, Benjamin and Mahmud, Samin Yaseer and Whitaker, Justin and Enck, William and Reaves, Bradley and Singh, Kapil and Egelman, Serge},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={985--1002},
  year={2020}
}

@inproceedings{andow2019policylint,
  title={$\{$PolicyLint$\}$: investigating internal privacy policy contradictions on google play},
  author={Andow, Benjamin and Mahmud, Samin Yaseer and Wang, Wenyu and Whitaker, Justin and Enck, William and Reaves, Bradley and Singh, Kapil and Xie, Tao},
  booktitle={28th USENIX security symposium (USENIX security 19)},
  pages={585--602},
  year={2019}
}

@inproceedings{zimmeck2016automated,
  title={Automated analysis of privacy requirements for mobile apps},
  author={Zimmeck, Sebastian and Wang, Ziqi and Zou, Lieyong and Iyengar, Roger and Liu, Bin and Schaub, Florian and Wilson, Shomir and Sadeh, Norman and Bellovin, Steven and Reidenberg, Joel},
  booktitle={2016 AAAI Fall Symposium Series},
  year={2016}
}

@inproceedings{bui2021consistency,
  title={Consistency analysis of data-usage purposes in mobile apps},
  author={Bui, Duc and Yao, Yuan and Shin, Kang G and Choi, Jong-Min and Shin, Junbum},
  booktitle={Proceedings of the 2021 ACM SIGSAC Conference on Computer and Communications Security},
  pages={2824--2843},
  year={2021}
}

@inproceedings{trimananda2022ovrseen,
  title={$\{$OVRseen$\}$: Auditing Network Traffic and Privacy Policies in Oculus $\{$VR$\}$},
  author={Trimananda, Rahmadi and Le, Hieu and Cui, Hao and Ho, Janice Tran and Shuba, Anastasia and Markopoulou, Athina},
  booktitle={31st USENIX security symposium (USENIX security 22)},
  pages={3789--3806},
  year={2022}
}

@inproceedings{liu2022promal,
  title={ProMal: precise window transition graphs for android via synergy of program analysis and machine learning},
  author={Liu, Changlin and Wang, Hanlin and Liu, Tianming and Gu, Diandian and Ma, Yun and Wang, Haoyu and Xiao, Xusheng},
  booktitle={Proceedings of the 44th International Conference on Software Engineering},
  pages={1755--1767},
  year={2022}
}

@inproceedings{liu2023ex,
  title={Ex pede Herculem: Augmenting Activity Transition Graph for Apps via Graph Convolution Network},
  author={Liu, Zhe and Chen, Chunyang and Wang, Junjie and Su, Yuhui and Huang, Yuekai and Hu, Jun and Wang, Qing},
  booktitle={2023 IEEE/ACM 45th International Conference on Software Engineering (ICSE)},
  pages={1983--1995},
  year={2023},
  organization={IEEE}
}

@article{arzt2014flowdroid,
  title={Flowdroid: Precise context, flow, field, object-sensitive and lifecycle-aware taint analysis for android apps},
  author={Arzt, Steven and Rasthofer, Siegfried and Fritz, Christian and Bodden, Eric and Bartel, Alexandre and Klein, Jacques and Le Traon, Yves and Octeau, Damien and McDaniel, Patrick},
  journal={Acm Sigplan Notices},
  volume={49},
  number={6},
  pages={259--269},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@article{enck2014taintdroid,
  title={Taintdroid: an information-flow tracking system for realtime privacy monitoring on smartphones},
  author={Enck, William and Gilbert, Peter and Han, Seungyeop and Tendulkar, Vasant and Chun, Byung-Gon and Cox, Landon P and Jung, Jaeyeon and McDaniel, Patrick and Sheth, Anmol N},
  journal={ACM Transactions on Computer Systems (TOCS)},
  volume={32},
  number={2},
  pages={1--29},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@inproceedings{shenao-2023,
author = {Wang, Shenao and Zhao, Yanjie and Wang, Kailong and Wang, Haoyu},
title = {On the Usage-Scenario-Based Data Minimization in Mini Programs},
year = {2023},
pages = {29–32},
series = {{SaTS}}
}

@Misc{frida,
  title = "{frida}",
  author="{frida}",
  note = {\url{https://github.com/frida/frida}},
  year=2023
}

